Novel constraints on fermionic dark matter from galactic observables I: The Milky Way

We have recently introduced a new model for the distribution of dark matter (DM) in galaxies based on a self-gravitating system of massive fermions at finite temperatures, the Ruffini-Arg\"uelles-Rueda (RAR) model. We show that this model, for fermion masses in the keV range, explains the DM halo of the Galaxy and predicts the existence of a denser quantum core at the center. We demonstrate here that the introduction of a cutoff in the fermion phase-space distribution, necessary to account for the finite Galaxy size, defines a new solution with a central core which represents an alternative to the black hole (BH) scenario for SgrA*. For a fermion mass in the range $mc^2 = 48$ -- $345$~keV, the DM halo distribution is in agreement with the Milky Way rotation curve data, while harbors a dense quantum core of about $4\times10^6 M_\odot$ within the S2-star pericenter.

==> figures/rhozoom/figure.tex <==
\begin{figure*}%
	\centering%
	\includegraphics[width=0.7\hsize,clip]{\ROOTPATH/fig.pdf}
	\caption{(Color online) Comparison of the density profile as given by the RAR model (for a fermion masses $m c^2=48$~keV and 345~keV) and the phenomenological NFW model (from \protect\citet{2013PASJ...65..118S}, but see also \protect\citet{2017PDU....15...90I} for the possible implementation of generalized NFW models) in the region $r = 2$ -- $40$~kpc. Note that curves for both RAR solutions coincide in the halo as shown here.}
	\label{fig:rhozoom}
\end{figure*}
